New Bounds on Optimal Sorting Networks

We present new parallel sorting networks for $17$ to $20$ inputs. For $17, 19,$ and $20$ inputs these new networks are faster (i.e., they require less computation steps) than the previously known best networks. Therefore, we improve upon the known upper bounds for minimal depth sorting networks on $17, 19,$ and $20$ channels. Furthermore, we show that our sorting network for $17$ inputs is optimal in the sense that no sorting network using less layers exists. This solves the main open problem of [D. Bundala & J. Za\'vodn\'y. Optimal sorting networks, Proc. LATA 2014].

==> drawnets.tex <==
\usepackage{tikz}
\usepackage[trim]{tokenizer} 
\usepackage{scalefnt}

\makeatletter

\newcounter{sncolumncounter}
\newcounter{snrowcounter}


\def \nodeconnection#1{%
  \foreach \i in {#1}{%
    \GetTokens{nodesrc}{nodedest}{\i}
    \draw (\value{sncolumncounter}/2,-\nodesrc) node[circle,inner sep=0pt,minimum size=3pt,fill=black]{}--(\value{sncolumncounter}/2,-\nodedest) node[circle,inner sep=0pt,minimum size=3pt,fill=black]{};
  }
  \addtocounter{sncolumncounter}{1}
}

\def \lnodeconnection#1{%
{\scalefont{0.5}
  \foreach \i in {#1}{%
    \GetTokens{nodesrc}{nodedest}{\i}
    \draw (\value{sncolumncounter}/2,-\nodesrc) node[circle,inner sep=0pt,minimum size=4pt,fill=black,label={[label distance=-3pt]45:$\text{out}_{\text{min}}$},label={[label distance=-3pt]135:$\text{in}_1$}]{}--(\value{sncolumncounter}/2,-\nodedest) node[circle,inner sep=0pt,minimum size=4pt,fill=black,label={[label distance=-3pt]45:$\text{out}_{\text{max}}$},label={[label distance=-3pt]135:$\text{in}_2$}]{};
    %\draw (\value{sncolumncounter}/2+0.2,-\nodesrc+0.2) node {test};
  }
  \addtocounter{sncolumncounter}{5}
  }
}

 
\newenvironment{sortingnetwork}[3]
{
  \setcounter{sncolumncounter}{0}
  \def \sn@fullsize{15}
  \begin{center}
  \begin{tikzpicture}[scale=.22]%[scale=#3*\sn@fullsize/#2]
  \foreach \i in {1, ..., #1}
  {
    \draw (-1,-\i)--((#2/1.7,-\i);
  }
}
{
  \end{tikzpicture}
  \end{center}
}


\newenvironment{inlinesortingnetwork}[3]
{
  \setcounter{sncolumncounter}{0}
  \def \sn@fullsize{15}
  \begin{tikzpicture}[scale=.25]%[scale=#3*\sn@fullsize/#2]
  \foreach \i in {1, ..., #1}
  {
    \draw (-1,-\i)--((#2/1.7,-\i);
  }
}
{
  \end{tikzpicture}
}

\makeatother



